Speech enhancement with frequency domain auto-regressive modeling

Speech applications in far-field real world settings often deal with signals that are corrupted by reverberation. The task of dereverberation constitutes an important step to improve the audible quality and to reduce the error rates in applications like automatic speech recognition (ASR). We propose a unified framework of speech dereverberation for improving the speech quality and the ASR performance using the approach of envelope-carrier decomposition provided by an autoregressive (AR) model. The AR model is applied in the frequency domain of the sub-band speech signals to separate the envelope and carrier parts. A novel neural architecture based on dual path long short term memory (DPLSTM) model is proposed, which jointly enhances the sub-band envelope and carrier components. The dereverberated envelope-carrier signals are modulated and the sub-band signals are synthesized to reconstruct the audio signal back. The DPLSTM model for dereverberation of envelope and carrier components also allows the joint learning of the network weights for the down stream ASR task. In the ASR tasks on the REVERB challenge dataset as well as on the VOiCES dataset, we illustrate that the joint learning of speech dereverberation network and the E2E ASR model yields significant performance improvements over the baseline ASR system trained on log-mel spectrogram as well as other benchmarks for dereverberation (average relative improvements of 10-24% over the baseline system). The speech quality improvements, evaluated using subjective listening tests, further highlight the improved quality of the reconstructed audio.

==> Tables/older_table.tex <==
\begin{table}[t!]
\centering
\caption{Comparison of the results with other works reported on the REVERB challenge dataset. }
\resizebox{0.94\columnwidth}{!}{%
\begin{tabular}{l|c|c|c}
\toprule
System & Eval-sim. & Eval-real & Avg. \\   \hline       
Subramanian et. al.~\cite{subramanian2019investigation} & 6.6 & 10.6 & 8.6 \\  
Heymann et. al.      & -              & 10.8  & - \\    
Fujita et. al.~\cite{fujita2020attention} & \textbf{4.9 }& 9.8 & 7.4\\ 
Purushothaman et. al.~\cite{purushothaman2022dereverberation} & 7.1 & 12.1 & 9.6 \\ 
Zhang et. al.~\cite{zhang2020end}      & -              & 10.0  & - \\  \midrule  
This work & 5.7  & \textbf{7.3} &\textbf{ 6.5} \\
\bottomrule
\end{tabular}}
\vspace{-0.2cm}
\label{table:reverb_Prior}
\end{table}
